Unintended memorisation of unique features in neural networks

Neural networks pose a privacy risk due to their propensity to memorise and leak training data. We show that unique features occurring only once in training data are memorised by discriminative multi-layer perceptrons and convolutional neural networks trained on benchmark imaging datasets. We design our method for settings where sensitive training data is not available, for example medical imaging. Our setting knows the unique feature, but not the training data, model weights or the unique feature's label. We develop a score estimating a model's sensitivity to a unique feature by comparing the KL divergences of the model's output distributions given modified out-of-distribution images. We find that typical strategies to prevent overfitting do not prevent unique feature memorisation. And that images containing a unique feature are highly influential, regardless of the influence the images's other features. We also find a significant variation in memorisation with training seed. These results imply that neural networks pose a privacy risk to rarely occurring private information. This risk is more pronounced in healthcare applications since sensitive patient information can be memorised when it remains in training data due to an imperfect data sanitisation process.

==> checklist.tex <==
\section*{Checklist}


%%% BEGIN INSTRUCTIONS %%%
The checklist follows the references.  Please
read the checklist guidelines carefully for information on how to answer these
questions.  For each question, change the default \answerTODO{} to \answerYes{},
\answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
justification to your answer}, either by referencing the appropriate section of
your paper or providing a brief inline description.  For example:
\begin{itemize}
  \item Did you include the license to the code and datasets? \answerYes{See Section \ref{gen_inst}.}
  \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
  \item Did you include the license to the code and datasets? \answerNA{}
\end{itemize}
Please do not modify the questions and only use the provided macros for your
answers.  Note that the Checklist section does not count towards the page
limit.  In your paper, please delete this instructions block and only keep the
Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%


\begin{enumerate}


\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    
  \answerYes{We show that unique feature memorisation occurs in neural networks. We evidence this using white box method and black box method. Our results are supported using significance testing (See Table \ref{table:memorisation-whitebox} and Table \ref{table:memorisation}). We describe a black box method for detecting feature memorisation in Section \ref{sec:method}. We show that regularisers do not eliminate memorisation in Section \ref{result:3} and we state which results are not statistically significant. Finally we describe which factors influence unique feature memorisation and support these findings with empirical results in Section \ref{sec:discussion}}
  \item Did you describe the limitations of your work?
  \answerYes{In Section \ref{sec:method} we make an assumption that we know the unique feature. We describe this assumption and enumerate some scenarios where knowing the unique feature is quite possible.}
  \item Did you discuss any potential negative societal impacts of your work?
  \answerNo{We do not believe our work has any potential negative societal impacts. On the contrary we believe our work illuminates privacy issues which occur in models already.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
  \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
  \answerNA{}
        \item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{We include an anonymous reference to an online repository containing all of the above in Section \ref{sec:models-and-training}.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{We include our training strategy in Section \ref{sec:models-and-training}.}
        \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{We report the statistical significance of $M$ using a t-test (See Table \ref{table:memorisation-whitebox} and Table \ref{table:memorisation}). In Section \ref{sec:models-and-training} we include experiments over multiple evaluations with error bars.}
        \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{We report on the above in Section \ref{sec:models-and-training}.}
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{We use existing datasets and models. We reference these correctly in Section \ref{sec:models-and-training}.}
  \item Did you mention the license of the assets?
    \answerYes{We mention the license of the assets that we use in Section \ref{sec:models-and-training}.}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNo{Yes we include new experiments as a PDF in the supplementary materials.}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerYes{All data was obtained from the public domain.}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerYes{In Figure \ref{fig:the-gist} we reference the source of an X-ray image. We use a fictional name and age superimposed on this image.}
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}
